Bootstrapping Motor Skill Learning with Motion Planning

Learning a robot motor skill from scratch is impractically slow; so much so that in practice, learning must be bootstrapped using a good skill policy obtained from human demonstration. However, relying on human demonstration necessarily degrades the autonomy of robots that must learn a wide variety of skills over their operational lifetimes. We propose using kinematic motion planning as a completely autonomous, sample efficient way to bootstrap motor skill learning for object manipulation. We demonstrate the use of motion planners to bootstrap motor skills in two complex object manipulation scenarios with different policy representations: opening a drawer with a dynamic movement primitive representation, and closing a microwave door with a deep neural network policy. We also show how our method can bootstrap a motor skill for the challenging dynamic task of learning to hit a ball off a tee, where a kinematic plan based on treating the scene as static is insufficient to solve the task, but sufficient to bootstrap a more dynamic policy. In all three cases, our method is competitive with human-demonstrated initialization, and significantly outperforms starting with a random policy. This approach enables robots to to efficiently and autonomously learn motor policies for dynamic tasks without human demonstration.

==> scraps.tex <==
%\banote{from talking to Nishanth: LfD = Imitation Learning. Two families of methods: 1) behavior cloning 2) IRL. 1) is tough because of brittleness, need lots of samples to cover state space. 2) is tough because RL is in the inner loop. We are a bit of a weird case because reward function exists.} \ernote{I think of our method as first performing supervised learning to learn a model-free mapping from state to actions (behavioral cloning), and then using reinforcement learning to further improve the model. Both components are grounded in kinematic descriptions of the robot and object.} 
%See the recent review \href{https://www.annualreviews.org/doi/pdf/10.1146/annurev-control-100819-063206}{here}. 
